The Role of Edges in Line Drawing Perception

It has often been conjectured that the effectiveness of line drawings can be explained by the similarity of edge images to line drawings. This paper presents several problems with explaining line drawing perception in terms of edges, and how the recently-proposed Realism Hypothesis of Hertzmann (2020) resolves these problems. There is nonetheless existing evidence that edges are often the best features for predicting where people draw lines; this paper describes how the Realism Hypothesis can explain this evidence.

==> The Role of Edges in Line Drawing Perception/texfigures_arxiv/david_nose.tex <==
\newcommand{\davidwide}{1.8in}
\newcommand{\davidnosewide}{1.8in}
\newcommand{\xwide}{1.8in}
\newcommand{\spw}{0in}

\begin{figure}
    \centering
    \begin{tabular}{c@{ }c@{ }c@{ }c@{ }}
        {{\sf A.} Headlight} &  
        {\textsf{ B.} Occluding} &
    {\textsf{ C.} Apparent Ridges} \\[-0.5ex]
{Rendering} & {+ Suggestive Contours} & \\
%
    \includegraphics[width=\davidwide]{figures/david/David_diffuse.jpg} &
    \includegraphics[width=\davidwide]{figures/david/David_SC.png} &
    \includegraphics[width=\davidwide]{figures/david/David_AR.png} \\
        \includegraphics[width=\davidnosewide]{figures/david/david_diffuse_nose2.pdf} &
    \includegraphics[width=\davidnosewide]{figures/david/David_SC_nose2.jpg} &
    \includegraphics[width=\davidnosewide]{figures/david/david_AR_nose2.pdf} \\[2ex]
    \textsf{ D}~~
    \includegraphics[width=\xwide]{figures/david/profile_diffuse.pdf}\hspace{\spw} &
    \textsf{ E}~~
    \includegraphics[width=\xwide]{figures/david/profile_sc.pdf}\hspace{\spw} &
    \textsf{ F}~~
    \includegraphics[width=\xwide]{figures/david/profile_ar.pdf}\hspace{\spw} \\
%\small{Ridges}
\end{tabular}
    \caption{Line drawing algorithms.
    Panels A, B, C: Three renderings of a 3D model.
    Panel D: possible cross-section of the 3D surface along the red line.
    Panels E, F: cross-sections of possible shape percepts of the drawings. There is an extra Apparent Ridge curve indicated by the red arrow. This curve on the nose may be perceived as a Suggestive Contour (SC) that implies a more pinched surface than the Suggestive Contour rendering does.
   (\href{https://www.myminifactory.com/object/3d-print-2052}{Model} by Scan The World, rendered with \href{https://github.com/fcole/qrtsc}{qrtsc} )
    }
    \label{fig:david_nose}
\end{figure}

==> The Role of Edges in Line Drawing Perception/texfigures_arxiv/david_rh.tex <==
%\newcommand{\dogheight}{1.3in}
%\newcommand{\davidlabel}[1]{\raisebox{\dogheight}{\textbf{\sf #1}}}
%\newcommand{\davidgap}{-0.15in}
%\newcommand{\davidgap}{-0.15in}
\begin{figure}
    \centering
    \davidlabel{A}\hspace{\davidgap}
    \includegraphics[height=\dogheight]{figures/david/David_glossified.jpg}~~
    \davidlabel{B}\hspace{\davidgap}
    \includegraphics[height=\dogheight]{figures/david/david_glossified_ridges.jpeg}
    \caption{
Renderings in the Realism Hypothesis.
        \textbf{Panel A:}
        A 3D model with a white satin material, viewed with headlight illumination.
        \textbf{Panel B:}
        Valleys of the realistic rendering, detected using a valley-detection algorithm, see \cite{Lee:2007}.
    \label{fig:david_rh}}
\end{figure}

==> The Role of Edges in Line Drawing Perception/texfigures_arxiv/davidlae.tex <==
\newcommand{\dogheight}{1.7in}
\newcommand{\davidlabel}[1]{\raisebox{\dogheight}{\textbf{\sf #1}}}
%\newcommand{\davidgap}{-0.15in}
\newcommand{\davidgap}{-0.15in}
\begin{figure}
    \centering
    \davidlabel{A}\hspace{\davidgap}
    \includegraphics[height=\dogheight]{figures/david/David_diffuse.jpg}\hfill
    \davidlabel{B}\hspace{\davidgap}
    \includegraphics[height=\dogheight]{figures/david/david_dog.jpeg}\hfill
    %\qquad    
    \davidlabel{C}\hspace{\davidgap}        \includegraphics[height=\dogheight]{figures/david/david_gallery.jpg}\hfill
        \davidlabel{D}\hspace{\davidgap}
\includegraphics[height=\dogheight]{figures/david/david_gallery_edges.jpg}
    %\davidlabel{C}\hspace{\davidgap}        \includegraphics[height=\dogheight]{figures/david/david_scene2.jpg}\hfill
    %    \davidlabel{D}\hspace{\davidgap}
%\includegraphics[height=\dogheight]{figures/david/david_scene2_edges.jpg}

    \caption{
Creating line drawings with edge detection.
        \textbf{Panel A:}
        A 3D model with white Lambertian material and headlight illumination.
        \textbf{Panel B:}
Edge detection on this image produces a plausible line drawing. 
 \textbf{Panel C:}
    Many realistic images contain contours that would not normally appear in a line drawing, due to effects like specular reflection, texture, and cast shadows. 
    \textbf{Panel D:} Edge detection on this image does not produce a plausible line drawing.
    (Edge images computed with Difference-of-Gaussians, see \cite{Marr:1980,Young};    
    \href{https://www.myminifactory.com/object/3d-print-2052}{Model} by Scan The World, \href{https://stock.adobe.com/images/interior-with-concrete-wall/303492332?asset_id=303492332}{background image} by peshkova)}
    \label{fig:davidLAE}
\end{figure}

==> The Role of Edges in Line Drawing Perception/texfigures_arxiv/drawings.tex <==
\newcommand{\drawwidth}{1.4in}

\begin{figure}
\textsf{A} \\
    %\includegraphics[width=\drawwidth]{figures/drawings/david-pencil-gray2.jpg}~~
       \includegraphics[width=\drawwidth]{figures/drawings/david-sketchy-pencil.jpg}\hfill
       \includegraphics[width=\drawwidth]{figures/drawings/david-sketchy-pencil2.jpg}\hfill
  %\includegraphics[width=\drawwidth]{figures/drawings/david-watercolor.jpg}~~
          \includegraphics[width=\drawwidth]{figures/drawings/david-oilpaint2.jpg}   \hfill
%\includegraphics[width=\drawwidth]{figures/drawings/david-paintcan.jpg}~~
     \includegraphics[width=\drawwidth]{figures/drawings/david-halftone.jpg}    \\[2ex]
     \textsf{B} \\
            \includegraphics[width=\drawwidth]{figures/drawings/edgeimages/edges-sketchy-pencil.jpg}\hfill
            \includegraphics[width=\drawwidth]{figures/drawings/edgeimages/edges-sketchy-pencil2.jpg}\hfill
  %\includegraphics[width=\drawwidth]{figures/drawings/edgeimages/edges2-watercolor.jpg}~~
          \includegraphics[width=\drawwidth]{figures/drawings/edgeimages/edges-oilpaint2.jpg}\hfill
     \includegraphics[width=\drawwidth]{figures/drawings/edgeimages/edges-halftone.jpg}  


    \caption{Different artistic styles can convey shape and appearance without preserving edges. Shading can convey tone that is not captured by edges. \textbf{Panel A:} Artistic renditions of the ``David'' model.  \textbf{Panel B:} Edges of the first row images. In each case, the parameters of the DoG filter were manually set to best capture the edges, with some cases using much larger blur factors than others, since it is unclear how to determine edge scale in Lines-As-Edges. Even when coarse-scale edges are preserved, the overall information contained in the image is different, especially with of shading. \label{fig:drawings}
}
\end{figure}

==> The Role of Edges in Line Drawing Perception/texfigures_arxiv/mooney.tex <==
%\newcommand{\mooneyheight}{1in}
\newcommand{\mooneyheight}{1.2in}

\begin{figure}
    \centering
    \textsf{A} 
    \includegraphics[width=\mooneyheight]{figures/mooney/U0496.jpg}~~
    \textsf{B} 
    \includegraphics[width=\mooneyheight]{figures/mooney/U0496-edges.jpg} ~~~~~~
    \textsf{C} 
    \includegraphics[width=\mooneyheight]{figures/mooney/U0497.jpg} ~~
    \textsf{D} 
    \includegraphics[width=\mooneyheight]{figures/mooney/U0497-edges.jpg}
%    \includegraphics[height=\mooneyheight]{figures/mooney/patio_stairs.jpg} ~~
%    \includegraphics[height=\mooneyheight]{figures/mooney/patio_stairs_edges.jpeg}
\caption{Lines-As-Edges treats lines and edges as perceptually-equivalent. Hence, according to Lines-As-Edges, the image in Panel A should give the same shape percept as Panel B, as should C and D.  (Images A and C from \cite{Mooney2}, CC-BY.) }
    \label{fig:mooney}
\end{figure}
